Unclonable Encryption, Revisited

Unclonable encryption, introduced by Broadbent and Lord (TQC'20), is an encryption scheme with the following attractive feature: given a ciphertext, an adversary cannot create two ciphertexts both of which decrypt to the same message as the original ciphertext. We revisit this notion and show the following: - Reusability: The constructions proposed by Broadbent and Lord have the disadvantage that they either guarantee one-time security (that is, the encryption key can only be used once to encrypt the message) in the plain model or they guaranteed security in the random oracle model. We construct unclonable encryption schemes with semantic security. We present two constructions (for public-key and private-key settings) from minimal cryptographic assumptions. - Lower Bound and Generalized Construction: We revisit the information-theoretic one-time secure construction of Broadbent and Lord. The success probability of the adversary in their construction was guaranteed to be $0.85^n$, where $n$ is the length of the message. It was interesting to understand whether the ideal success probability of (negligibly close to) $0.5^n$ was unattainable. We generalize their construction to be based on a broader class of monogamy of entanglement games. We demonstrate a simple cloning attack that succeeds with probability $0.71^n$ against a class of schemes including that of Broadbent and Lord. We also present a $0.75^n$ cloning attack exclusively against their scheme. - Implication to Copy-Protection: We show that unclonable encryption, satisfying a stronger property, called unclonable-indistinguishability (defined by Broadbent and Lord), implies copy-protection for a simple class of unlearnable functions. While we currently don't have encryption schemes satisfying this stronger property, this implication demonstrates a new path to construct copy-protection.

==> ideas.tex <==
\section{Ideas for future work (Not part of the submitted version).}

\subsection{Construction of unclonable-Indistinguishable Secure Encryption}
unclonable Indistinguishable Security \cite{BL19} states that $\bob$ and $\charlie$ cannot simultaneously distinguish between encryptions of $m_0$ and $m_1$. \\ \\
\noindent Public-key encryption resilient to key-leakage attacks. \cite{NaorSegev09} shows constructions resilient to leakage of $L(1 - o(1))$ bits of the key, where $L$ is the key length.
\paragraph{Construction:} Let $\ue$ be an unclonable-encryption scheme and let $\pke$ be a public-key encryption scheme resilient to key leakage (Definition 3.1 in \cite{NaorSegev09}, Chosen-Plaintext Leakage Attack). \begin{itemize}
    \item{\bf Setup:} $k_\ue \leftarrow \ue.\gen(1^\secparam)$

    \item{\bf Encryption:} To encrypt a message $m$ with key $k_\ue$, first sample $(pk, sk) \leftarrow \pke.\gen(1^\secparam)$, then output $(\ue.\enc(k_{\ue}, sk), \pke.\enc(pk, m), pk)$
    
\end{itemize}

\paragraph{Correctness.}

\paragraph{Security.}(Intuition) either $\bob$ or $\charlie$ will recover less than $L(1 - o(1))$ bits of $sk$, meaning they cannot break semantic security of $\pke$. 
\begin{itemize}
    \item Given one of Bob's or Charlie's state, first lower bound the entropy of the secret key in the unclonable encryption scheme. Let's say the lower bound is $X$. [TRICKY] \prab{for Tuesday} \begin{itemize}
        \item In the $\ue$ cloning experiment without the public key, either Bob or Charlie has min-entropy at least\footnote{Approximation $\log(.85)\approx-1/4$ is being used.} $n/8 - \epsilon/2$, where $n = |sk|$ and $h = n - \epsilon = H_{\min}(sk)$.
        \item When the public key is known, we can argue that min-entropy of $sk$ changes by a small amount, since $pk$ should not reveal $sk$.
        \item In particular, if $\pke$ satisfies $H_{\min}(sk \given pk) = n - o(n)$, then either Bob or Charlie has min-entropy at least $n/8 - o(n)$.
    \end{itemize}
    \item Come up with a secret key encryption scheme that is scure even if the entropy of the secret key is $X$. We need to make sure that this is secure if the auxiliary information is quantum. 
    \item Assuming that the secret key encryption is secure, show that the above scheme satisfies UE-indistinguishability property. \prab{for Tuesday} 
\end{itemize}




\subsection{To-Do}
\begin{itemize}
%\item \textbf{TQC Comment:} Mention that the (second) ROM construction of Broadbent and Lord satisfies CPA security.
%\item \textbf{Check whether copy detection in \cite{ALLZZ20} implies copy protection.}
\item Construct copy protection with computational/correctness
%\item Quantum CCA Security
\item Upgrade to regular correctness (bounded correctnes one-way hash functions, 
\item Construct unclonable encrtyption assuming computational copy-protection (cannot copy with computational correctness) of function families with $\secparam$-bit key entropy.\footnote{Pairwise ind. < universal one-way < collision-res.} and a collision resistant hash function $H$ mapping $2\secparam$ bits to $\secparam$ bits. (ciphertext includes the copy-protected point function $f_{k,m}$ as well as hash of the key $H(k)$).  
\item Show that private-key UE satisfies many-time uncloneability.
\item Does unclonable encryption imply infinite-term SSL or copy detection?
\item unclonable-indistinguishable security implies copy-protection.
\item Cite \cite{hiroka2021quantum} and \cite{cryptoeprint:2021:408} as concurrent work
%\item remove $\secparam$ from conjugate encryption.
\item Strong unforgeability suffices (instead of unique signatures).
\end{itemize}
